VRAG-DFD: Verifiable Retrieval-Augmentation for MLLM-based Deepfake Detection

In Deepfake Detection (DFD) tasks, researchers proposed two types of MLLM-based methods: complementary combination with small DFD detectors, or static forgery knowledge injection. The lack of professional forgery knowledge hinders the performance of these DFD-MLLMs. To solve this, we deeply considered two insightful issues: How to provide high-quality associated forgery knowledge for MLLMs? AND How to endow MLLMs with critical reasoning abilities given noisy reference information? Notably, we attempted to address above two questions with preliminary answers by leveraging the combination of Retrieval-Augmented Generation (RAG) and Reinforcement Learning (RL). Through RAG and RL techniques, we propose the VRAG-DFD framework with accurate dynamic forgery knowledge retrieval and powerful critical reasoning capabilities. Specifically, in terms of data, we constructed two datasets with RAG: Forensic Knowledge Database (FKD) for DFD knowledge annotation, and Forensic Chain-of-Thought Dataset (F-CoT), for critical CoT construction. In terms of model training, we adopt a three-stage training method (Alignment->SFT->GRPO) to gradually cultivate the critical reasoning ability of the MLLM. In terms of performance, VRAG-DFD achieved SOTA and competitive performance on DFD generalization testing.

==> sec/_1__intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets the figure captions and references in a smaller font.
The reason why such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The review process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in 11 pages.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler that should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use the options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Use fractional references (\eg, this line is $087.5$), although in most cases the approximate location would be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please, number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for the reader to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean that some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not mean that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of our previous paper [1], and show that it is inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of the paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time that covers similar or overlapping material, you may need to refer to that submission to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, do not assume that the reviewers will read this material.

Sometimes your paper is about a problem that you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think that it is likely that the new article was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
However, for your results, you should not identify yourself and should not mention your participation in the challenge.
Instead, present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison with other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has only two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/_2__formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
The columns should be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered, and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

The captions of the figures and tables should be in 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centered.  Table captions should be above tables, while figure captions should be below figures.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period, and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use the footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example, at the beginning of the sentence, you can use
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, include the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When citing multiple papers at once, make sure that you cite them in numerical order such as this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \caption{Results.   Ours is better.}
  \label{tab:example}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead, use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise and, therefore, must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence, avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/_3__finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/prompts/full.tex <==
\section{Examples of full prompt}
Taking the assessment of color consistency as an example, the process begins with GPT-4V analyzing video frames to generate initial descriptions, followed by two specialized assistants that ask a ``chain'' of questions on object-color accuracy and color relationships respectively. Then MLLM answers these questions.
% 
The scoring process is assigning a 3-point color consistency score based on synthesized descriptions and video verification.

\clearpage
\onecolumn
\label{sec:example_of_full_prompt}
\paragraph{Video description}
To systematically evaluate color consistency, we design a specialized prompt for GPT-4V(ision) that instructs the model to analyze color-related attributes in videos. Taking video frames as input, the model generates both a concise caption and a detailed description, specifically analyzing color stability, sudden changes, object-background color relationships, and proper color classification under various lighting conditions. The following shows our carefully engineered system prompt:
\begin{minted}[fontsize=\footnotesize]{python}

<instructions>
### Task Description:
"""You are a video description expert, you need to focus on describing the colors in the video. You will receive an AI-generated video. 
Your task is to carefully watch the video and provide a detailed description of the color conditions present in the video according to the "Describing Strategy" outlined below."""

### Important Notes:
"""1.Whether there is a sudden change in the color of the background or the color of the object.
2.Is there a single color or multiple colors on the object.
3.Whether the color of the object is very close to or even blends with the color of a part of the background?
4.Color changes due to sunlight exposure are not considered color mutations.
5.When the objec's color appears as dark blue, dark green, or other colors close to black due to lighting or other factors, the object's original color should be considered black.
6.When the color of an object appears as light gray, off-white, or similar shades close to white due to lighting angles or other factors, the object should be considered as originally being white."""

### Describing Strategy:
"""Your description must focus on the color situation in the video. Please follow these steps:
1. Observe and identify the object in the video.
2. Carefully observe all the colors on the object, including the proportion of each color and the stability of the colors. Also describe the colors of the background and their stability. Notice Whether the object's color is very close to or even blends with the color of a part of the background.
3. Give a description of the entire video based on above observations.
4. generate a one-sentence caption summarizing the colors of the object in the video."""

### Output Format:
"""For caption, use the header "[Caption]:" to introduce the caption.
For description, use the header "[Video Description]:" to introduce the description."""

<example>
[Video Caption]:
(Here, describe the caption.)

[Video Description]:
(Here, describe the entire video.)
</example>

</instructions>

\end{minted}

\paragraph{Chain of query}
The evaluation assistant analyzes the consistency among text prompts, video descriptions, and concise captions, focusing on three dimensions: object recognition accuracy, color fidelity, and temporal color stability. When discrepancies are detected, the assistant raises specific questions. The following shows the prompt design for the evaluation assistant:
\begin{minted}[fontsize=\footnotesize]{python}

### Task Description:
"""You are an evaluation assistant whose role is to help the leader reflect on its descriptions of the generated video. 
You need to carefully observe whether objects in the video can be recognized and consistent with the text prompt, whether colors in the video change abruptly and whether object's color in the video are consistent with the text prompt.
Your task is to identify the differences in object accuracy, color accuracy and stability between the caption, video description, and text prompt.
You need to ask questions that highlight these differences. If these differences do not appear, do not ask questions."""

### Important Notes: 
"""1. Focus on whether the generated object is correct. If the video description doesn't indicate what the object is, you must ask.
2. Focus on Whether the color of the object is consistent with the color in the text prompt.
3. Focus on whether the color remains stable throughout the video (Color changes due to sunlight exposure are not considered color mutations.)
4. Your question must highlight specific differences where the color in the video does not match the text prompt, as shown in the example."""

### Questioning Strategy:
"""Based on the video caption and video description, compare it to the text prompt's object and color requirements. 
You're only allowed two questions at most. If there's no question, you can say I don't have a question.
Your questions must follow these strategies:
Your question must highlight specific differences where the color in the video does not match the text prompt, as shown in the example.

1. Does the generated object in the video consistent with the object in the text prompt?
2. Can the color of the object in the video be considered the color of the text prompt?
3. Whether there are sudden changes in colors in the video?

Example Questions:
"Whether the object in the video can be recognized?"
"Whether the object in the video is a round object or a clock of the text prompt?"
“Can the orange color of the cat in the video be considered the yellow color of the text prompt?”
“Whether there are sudden changes in colors in the video?"""

### Output Format:
"""You need to first analyze if there are any differences in object accuracy, color accuracy and stability between the caption, video description and the text prompt, and then decide whether to ask questions.
Your response should follow the format given in the example."""

<example>
[Your analysis]:
(Your analysis should be here)

[Your question]:
<question>
question:... 
I have no question.
</question>
</example>
\end{minted}
The second evaluation assistant examines two specific aspects of color relationships: the presence of additional colors beyond those specified in the text prompt, and the color contrast between objects and backgrounds. The following shows the prompt design for the second evaluation assistant:
\begin{minted}[fontsize=\footnotesize]{python}
### Task Description:
"""
You are an evaluation assistant whose role is to help the leader reflect on its descriptions of the generated video. 
Your task is to identify the differences between caption, video description, and text prompt, including whether there are other colors on the object except the color in the text prompt, or Whether the object's color is close to the background's color.
You need to ask questions that point out these differences. If these differences do not appear, do not ask questions."""

### Important Notes:
"""1. Focus on Whether there are other colors on the object except the color in the text prompt.
2. Focus on Whether the object's color is very close to the background's color."""

### Questioning Strategy:
"""Based on the video caption and video description, compare it to the text prompt's color requirements. 
You're only allowed two questions at most. If there's no question, you can say I don't have a question.
Your questions must follow these strategies:
Your question must highlight specific differences where the color in the video does not match the text prompt, as shown in the example.

1. Whether other colors will affect the dominance of the required color of the text prompt?
2. Whether the color of the object is very close to the color of a part of the background?

Example Questions:
"The belly of the bird in the video is white, how much white occupies the area?"
"at first glance, the required color is the main color?
“The color of the object and the background are close, does the object's color blend into the background's color due to color similarity?"""

### Output Format:
"""You need to first analyze whether there are other colors on the object except the color in the text prompt, or whether the object's color is close to the background's color, and then decide whether to ask questions.
Your response should follow the format given in the example."""

<example>
[Your analysis]:
(Your analysis should be here)

[Your question]:
<question>
question:... 
I have no question.
</question>

</example>
\end{minted}

\paragraph{Chain of answer}
The final evaluator synthesizes observations and addresses questions raised by the previous assistants. It provides detailed descriptions focusing on object recognition, color accuracy, temporal stability, color distribution, and object-background relationships. Based on comprehensive analysis of the text prompt and video content, it resolves potential discrepancies identified in earlier stages. The following shows the prompt design for the final evaluator:
\begin{minted}[fontsize=\footnotesize]{python}
### Task Description:
"""You are now a Video Evaluation Expert. Your task is to carefully watch the text prompt and video carefully, describe the color in the video in detail and then evaluate the consistency between the video and the text prompt.
Your description must include whether the generated object can be recognized, whether the color is correct or similar, Whether there is a sudden change in the color in the video, how much area the other colors occupy the object, and whether they affect the dominance of the colors in the text prompt, and Whether the color of the object is very close to or even blends with the color of a part of the background?
When the assumptions in the assistants' question do not align with the text prompt, you need to carefully review the video, analyze the reasons for the discrepancy, and provide your judgement.
After you give the description and evaluation, please proceed to answer the provided questions."""

### Important Notes:
"""1. When the assumption in the question does not align with the text prompt, you need to carefully watch the video and think critically..
2. Your description must include the content mentioned in the "Task Description".
3. Whether the color of the object is very close to or even blends with the color of a part of the background?
4. Color changes due to sunlight exposure are not considered color mutations.
5. You must first give the description and evaluation before answering the questions."""

### Output Format:
"""You need to provide a detailed description and evaluation, followed by answering the questions.
For description, use the header "[Descriptions]:" to introduce the description and evaluation.
For the answers, use the header "[Answers]:" to introduce the answers.

<example>
[Descriptions]:
(Here, provide a detailed description of the video and evaluation, focusing on the color conditions.)

[Answers]:
(Here, answer the questions.)
</example>"""

### Evaluation Steps:
"""Follow the following steps strictly while giving the response:
1. Carefully read the "Task Description" and "Important Notes".
2. Carefully watch the text prompt and the video, then provide a detailed description and evaluate their consistency. 
3. Answer the provided questions.
4. Display the results in the specified 'Output Format'."""
\end{minted}

\paragraph{Final scoring}
Taking two independent video descriptions as input, this evaluator first synthesizes an updated description and then assigns scores on a 3-point scale. The scoring criteria specifically examine color accuracy, temporal stability, color distribution, and object-background relationships. Scores range from 1 (poor consistency) to 3 (good consistency), with detailed conditions defining moderate consistency (score 2). The following shows the prompt design for the scoring system:
\begin{minted}[fontsize=\footnotesize]{python}
### Task Description:
"""You are now a Video Evaluation Expert responsible for evaluating the consistency between AI-generated video and the text prompt. 
You will receive two video informations. The first one is an objective description based solely on the video content without considering the text prompt.
The second description will incorporate the text prompt. You need to carefully combine and compare both descriptions and provide a final, accurate updated video description based on your analysis.
Then, you need to evaluate the video's consistency with the text prompt based on the updated video description according to the instructions. 

<instructions>"""
### Evaluation Criteria:
"""You are required to evaluate the color consistency between the video and the text prompt.
Color consistency refers to the consistency in color between the video and the provided text prompt.
About how to evaluate this metric,after you watching the frames of videos,you should first consider the following:
1. Whether the color is consistent with the text prompt and remain consistent throughout the entire video and there are no abrupt changes in color.
2. Whether the color is on the right object or background.
3. Whether the colors are similar but not exactly the same?"""

### Scoring Range
"""Then based on the above considerations, you need to assign a specific score from 1 to 3 for each video(from 1 to 3, with 3 being the highest quality,using increments of 1) according to the 'Scoring Range':

1. Poor consistency - The generated object is incorrect or cannot be recognized or the color on the object does not match the text prompt at all.(e.g., yellow instead of red).
2. Moderate consistency - The correct color appears in the video, but it's not perfect. The specific conditions are:
    - Condition 1 : Incorrect color allocation, such as the color appearing in the background instead of on the object.
    - Condition 2 : Color instability, with sudden or fluctuating changes in the color on the object.
    - Condition 3 : Color confusion, where part of the object has the correct color but other color occupy a large area (at first glance, the required color is not the main color). (e.g., a white vase is generated as a black and white striped vase.)
    - Condition 4 : The object's color blends into the background color, making it difficult to distinguish.
    - Condition 5 : Similar color, the object's color is in the same color spectrum as the requested color but not very accurate. (e.g., pink instead of purple, or yellow instead of orange.)
3.  Good consistency  - The color is highly consistent with the text prompt, the color in the entire video is stable, the color distribution is correct, there are no sudden changes or inconsistencies in color, and there are no issues mentioned in the moderate consistency category."""

###Important Notes:
"""And you should also pay attention to the following notes:
1.The watermark in the video should not be a negative factor in the evaluation.
2.When the objec's color appears as dark blue, dark green, or other colors close to black due to lighting or other factors, the object's original color should be considered black.
4.When the color of an object appears as light gray, off-white, or similar shades close to white due to lighting angles or other factors, the object should be considered as originally being white.
3.Before assigning a 1 or 2 score, ensure you have reviewed the color spectrum and the conditions listed under moderate consistency. If the color is close but not perfect, consider whether it might fit under moderate consistency (2 points).  """        

### Output Format:
"""For the updated video description, you need to integrate the initial observations and feedback from the assistants and use the header "[updated description]:" to introduce the integrated description.
For the evaluation result, you should assign a score to the video and provide the reason behind the score and use the header "[Evaluation Result]:" to introduce the evaluation result.

<example>
[Updated Video Description]:
(Here is the updated video description)

[Evaluation Result]:
([AI model's name]: [Your Score], because...)
</example>"""

### Evaluation Steps:
"""Follow the following steps strictly while giving the response:
1.Carefully review the two informations, think deeply, and provide a final, accurate description.
2.Carefully review the "Evaluation Criteria" and "Important Notes." Use these guidelines when making your evaluation.
3.Score the video according to the "Evaluation Criteria" and "Scoring Range."
4.Display the results in the specified "Output Format."
</instructions>"""
\end{minted}

% \paragraph{Score refinement}
% A refined scoring mechanism evaluates color consistency between video generations and text prompts. It takes three inputs: an objective video description, a prompt-aware description, and the input video itself for verification.
% \begin{minted}[fontsize=\footnotesize]{python}
% ### Task Description:
% """You are now a Video Evaluation Expert responsible for evaluating the consistency between AI-generated video and the text prompt. 
% You will receive two video informations and a input video. The first one is an objective description based solely on the video content without considering the text prompt. 
% The second description will incorporate the text prompt. You need to carefully combine and compare both descriptions and provide a final, accurate updated video description based on your analysis. 
% You can verify the updated description with the video, and if it doesn't match the video, you can modify the updated description.
% Then, you need to evaluate the video's consistency with the text prompt based on the updated video description and the input video according to the instructions. 

% <instructions>"""
% ### Evaluation Criteria:
% """You are required to evaluate the color consistency between the video and the text prompt.
% Color consistency refers to the consistency in color between the video and the provided text prompt.
% About how to evaluate this metric,after you watching the frames of videos,you should first consider the following:
% 1. Whether the color is consistent with the text prompt and remain consistent throughout the entire video and there are no abrupt changes in color.
% 2. Whether the color is on the right object or background.
% 3. Whether the colors are similar but not exactly the same?"""

% ### Scoring Range
% """Then based on the above considerations, you need to assign a specific score from 1 to 3 for each video(from 1 to 3, with 3 being the highest quality,using increments of 1) according to the 'Scoring Range':

% 1. Poor consistency - The generated object is incorrect or cannot be recognized or the color on the object does not match the text prompt at all.(e.g., yellow instead of red).
% 2. Moderate consistency - The correct color appears in the video, but it's not perfect. The specific conditions are:
%     - Condition 1 : Incorrect color allocation, such as the color appearing in the background instead of on the object.
%     - Condition 2 : Color instability, with sudden or fluctuating changes in the color of the video.
%     - Condition 3 : Color confusion, where part of the object has the correct color but other color occupy a large area (at first glance, the required color is not the main color). (e.g., a white vase is generated as a black and white striped vase.)
%     - Condition 4 : The object's color blends into the background color, making it difficult to distinguish.
%     - Condition 5 : Similar color, the object's color is in the same color spectrum as the requested color but not very accurate. (e.g., pink instead of purple, or yellow instead of orange.)
%     - Condition 6 : The video contains multiple correctly generated objects, where some have the correct color while others do not (e.g., the text prompt is for a yellow box, and the video shows a yellow box and a green box).
% 3.  Good consistency  - The color is highly consistent with the text prompt, the color in the entire video is stable, the color distribution is correct, there are no sudden changes or inconsistencies in color, and there are no issues mentioned in the moderate consistency category."""

% ###Important Notes:
% """And you should also pay attention to the following notes:

% 1.The watermark in the video should not be a negative factor in the evaluation.
% 2.When the objec's color appears as dark blue, dark green, or other colors close to black due to lighting or other factors, the object's original color should be considered black.
% 4.When the color of an object appears as light gray, off-white, or similar shades close to white due to lighting angles or other factors, the object should be considered as originally being white."""

% ### Output Format:
% """For the updated video description, you need to integrate the initial observations and feedback from the assistants and use the header "[updated description]:" to introduce the integrated description.
% For the evaluation result, you should assign a score to the video and provide the reason behind the score and use the header "[Evaluation Result]:" to introduce the evaluation result.

% <example>
% [Updated Video Description]:
% (Here is the updated video description)

% [Evaluation Result]:
% ([AI model's name]: [Your Score], because...)
% </example>"""

% ### Evaluation Steps:
% """Follow the following steps strictly while giving the response:
% 1.Carefully review the two informations, think deeply, and provide a final, accurate description. 
% 2.Carefully watch the input video to verify the the updated description. If it doesn't match the video, you can modify the updated description.
% 3.Carefully review the "Evaluation Criteria", the "Important Notes" . Use these guidelines when making your evaluation.
% 4.Score the video according to the "Evaluation Criteria" and "Scoring Range."
% 5.Display the results in the specified "Output Format."
% </instructions>"""
% \end{minted}


% A score validation assistant is designed to verify and potentially adjust the initial consistency scores. Taking the text prompt and initial score as inputs, it ensures adherence to a 5-point scoring criteria that evaluates overall video-text consistency. The validation focuses on the presence and quality of core elements (subjects, objects, actions, scenes) and visual quality, with scores ranging from 1 (very poor consistency) to 5 (excellent consistency). The following shows the prompt design for the score validation system:
% \begin{minted}[fontsize=\footnotesize]{python}
% scorechecker_prompt = {
% "scorechecker":"""
% ### Task Description:
% You are now a Score Validation Assistant. You will receive a text prompt and a score for the video generated by the video generation model. 
% Your responsibility is to verify the score assigned by the AI model and ensure that it strictly adheres to the provided 'Evaluation Criteria' and 'Scoring Range'. 
% If the score does not match the 'Scoring Range', you must adjust it accordingly and provide reasoning for any score modifications based on the 'Scoring Range'.

% ### Evaluation Criteria:
% The AI model need to assess the overall consistency between the video and the text prompt. Overall consistency refers to how well the video content and style match the provided text prompt. When evaluating this metric, consider the following:
% 1. Does the video display all the core elements mentioned in the text prompt? (Core elements include subjects, objects, actions, scenes, numerical relationships, styles, spatial relationships, etc.)

% ### Scoring Range
%  Ensure the assigned score for each video falls within the following range, from 1 to 5 (with 5 being the highest quality), based strictly on the 'Evaluation Criteria':
% -1: Very poor consistency- more than half of the key elements, and the consistency is very weak,or the visual quality is too poor to understand the video.
% -2: Poor consistency- The video includes most of the key elements, but the generation of elements is not sufficient,or the visual quality is not good enough  to judge if the video is consitent with the text prompt.
% -3: Moderate consistency- The video includes most of the key elements and no element is not sufficiently generated, or the video includes all elements but most of them are not sufficiently generated.And the visual quality is good enough to judge if the video is consitent with the text prompt.
% -4: Good consistency- The video includes all key elements, with some elements not sufficiently generated.And the visual quality is good enough to judge if the video is consitent with the text prompt.
% -5: Excellent consistency- The video includes all of the key elements without elements not sufficiently generated and is perfectly consitent with the text prompt.And the visual quality is good enough to judge if the video is consitent with the text prompt.

% ### Output Format:
% After validating the score, use the header "[Updated Evaluation Result]:" to provide the result.

% <example>
% [Evaluation Result]:
% ([AI model's name]: [Updated Score], because...)
% </example>
% """
% }
% \end{minted}
\twocolumn

==> sec/table/ablation_.tex <==
% \begin{table*}[htbp]
%     \caption{
%     \textbf{Ablation study of RAG.}}
%     \centering
% \scriptsize

% \renewcommand\arraystretch{1.2}
% \small
% \centering
% \hspace*{0.00000000000000001cm}
%     \begin{subtable}[t]{0.4\textwidth}  % 左侧子表格
%     \renewcommand\tabcolsep{1pt}
%         \centering
%         \begin{tabular}{c|ccccc}
%             \hline

%             \hline

%             \hline

%             \hline
            
%             \multirow{2}*{Dataset} &\multicolumn{7}{c|}{\underline{\textit{\textbf{Test Set AUC}}}} & \\

%             & & FF++  & CDF1 & CDF2 & DFDC & FFIW & WDF & DFD  \\
%             \hline
            
%             \hline
%              &  $0.639$ & $0.627$ & $0.526$&$0.452$ & $0.561$ \\
%              \checkmark &  $\textbf{0.733}$ &$\textbf{0.702}$&$\textbf{0.531}$ &$\textbf{0.514}$ & $\textbf{0.620}$\\
%              \hline

%             \hline
                
%             \hline
                
%             \hline
%         \end{tabular}
%         \label{tab:RAG-abla}
%     \end{subtable}
%     \hfill
%     \begin{subtable}[t]
%     {0.54\textwidth}  % 右侧子表格
%         \renewcommand\tabcolsep{1pt}
%         \centering
%         \caption{
%         \textbf{Ablation study of Effort.}}
%         \begin{tabular}{c|cccccc}
%             \hline

%             \hline

%             \hline

%             \hline
            
%             \multirow{2}*{Dataset} &\multicolumn{7}{c|}{\underline{\textit{\textbf{Test Set AUC}}}} & \\

%             & & FF++  & CDF1 & CDF2 & DFDC & FFIW & WDF & DFD  \\
%             \hline
            
%             \hline
%               &$0.671$ &$0.690$ &$0.699$ & $0.662$&$0.675$ &$0.679$\\
%              \checkmark&$\textbf{0.732}$&$\textbf{0.735}$ & $\textbf{0.750}$&$\textbf{0.718}$ &$\textbf{0.733}$ & $\textbf{0.7336}$\\
%              \hline

%             \hline
                
%             \hline
                
%             \hline
%         \end{tabular}
%         \label{tab:effort-abla}
%     \end{subtable}

%     \label{tab:ablation-two-tables}
% \end{table*}


% \begin{table*}[htbp]
%     \centering
%     \scriptsize
%     \renewcommand\arraystretch{1.2}

%     % 左侧子表格
%     \begin{subtable}[t]{0.45\textwidth}  
%         \centering
%         \caption{\textbf{Ablation study of RAG.}}
%         \renewcommand\tabcolsep{2pt}
%         \begin{tabular}{c|cccccc}
%             \hline
%             \multirow{3}*{Metrics} & \multicolumn{6}{c}{\underline{Test Set AUC}} \\
            
%              & FF++ & CDF1 & CDF2 & DFDC & FFIW & WDF \\
%             \hline
%             MLLM & 0.639 & 0.627 & 0.526 & 0.452 & 0.561 & - \\
%             MLLM(w/RAG) & \textbf{0.733} & \textbf{0.702} & \textbf{0.531} & \textbf{0.514} & \textbf{0.620} & - \\
%             \hline
%         \end{tabular}
%         \label{tab:RAG-abla}
%     \end{subtable}
%     \hfill
%     % 右侧子表格
%     \begin{subtable}[t]{0.53\textwidth}  
%         \centering
%         \caption{\textbf{Ablation study of Effort.}}
%         \renewcommand\tabcolsep{2pt}
%         \begin{tabular}{c|cccccc}
%             \hline
%            \multirow{3}*{Metrics} & \multicolumn{6}{c}{\underline{Test Set AUC}} \\
            
%              & FF++ & CDF1 & CDF2 & DFDC & FFIW & WDF \\
%             \hline
%             CLIP & 0.639 & 0.627 & 0.526 & 0.452 & 0.561 & - \\
%             Effort & \textbf{0.733} & \textbf{0.702} & \textbf{0.531} & \textbf{0.514} & \textbf{0.620} & - 
%             \\
%             \hline
%         \end{tabular}
%         \label{tab:effort-abla}
%     \end{subtable}

%     % \caption{\textbf{Ablation studies of RAG and Effort.} Two sub-tables are placed side by side for comparison.}
%     \label{tab:ablation-two-tables}
% \end{table*}


% \begin{table*}[htbp]
%     \centering
%     \scriptsize
%     \renewcommand\arraystretch{1.2}

%     % 左侧子表格
%     \begin{subtable}[t]{0.45\textwidth}  
%         \centering
%         \caption{\textbf{Ablation study of stages.}}
%         \renewcommand\tabcolsep{2pt}
%         \begin{tabular}{c|cccccc}
%             \hline
%             \multirow{3}*{Metrics} & \multicolumn{6}{c}{\underline{Test Set AUC}} \\
            
%              & FF++ & CDF1 & CDF2 & DFDC & FFIW & WDF \\
%             \hline
%             stage1 & 0.639 & 0.627 & 0.526 & 0.452 & 0.561 & - \\
%             stage2(w/sft) & \textbf{0.733} & \textbf{0.702} & \\
%             stage3(w/sft+rl) & \textbf{0.733} & \textbf{0.702} &
%             \textbf{0.531} & \textbf{0.514} & \textbf{0.620} & - \\
%             \hline
%         \end{tabular}
%         \label{tab:stages-abla}
%     \end{subtable}
%     \hfill
%     % 右侧子表格
%     \begin{subtable}[t]{0.53\textwidth}  
%         \centering
%         \caption{\textbf{Ablation study of different MLLM.}}
%         \renewcommand\tabcolsep{2pt}
%         \begin{tabular}{c|cccccc}
%             \hline
%            \multirow{3}*{Metrics} & \multicolumn{6}{c}{\underline{Test Set AUC}} \\
            
%              & FF++ & CDF1 & CDF2 & DFDC & FFIW & WDF \\
%             \hline
%             Qwen2.5VL-7b & 0.639 & 0.627 & 0.526 & 0.452 & 0.561 & - \\
%             InternVL3-8b & \textbf{0.733} & \textbf{0.702} & \textbf{0.531} & \textbf{0.514} & \textbf{0.620} & - 
%             \\
%             \hline
%         \end{tabular}
%         \label{tab:MLLM-abla}
%     \end{subtable}

%     % \caption{\textbf{Ablation studies of RAG and Effort.} Two sub-tables are placed side by side for comparison.}
%     \label{tab:ablation-two-tables}
% \end{table*}

% -----------------------------------------------------
% 请确保在你的 LaTeX 导言区 (document 之前) 包含了以下宏包:
% \usepackage{caption}  % <- 这是实现独立编号的关键
% \usepackage{multirow}
% \usepackage{booktabs} % 推荐
% -----------------------------------------------------

\begin{table*}[htbp]
    \centering
    \scriptsize
    \renewcommand\arraystretch{1.2}

    % --------------------
    % 表 1 (左侧)
    % --------------------
    \begin{minipage}[t]{0.45\textwidth}
        \centering
        \captionsetup{type=table} % 关键: 告诉 LaTeX 这是一个独立的表格
        \caption{\textbf{Ablation study of RAG (AUC \%). 'w/o RAG' removes the forensic retriever and all associated critical reasoning components. }}
        \label{tab:abla-RAG} % 更改了标签以防冲突
        \renewcommand\tabcolsep{2pt}
        \begin{tabular}{c|cccccc}
            \hline
            \multirow{2}*{Metrics} & \multicolumn{5}{c}{\underline{Test Set AUC}} \\
             & CDF1 & CDF2 & DFDC & FFIW & WDF \\
            \hline
            w/o RAG Module & 91.13 & 87.85 & 72.42 & 78.62 & 71.62  \\
            VRAG-DFD & \textbf{99.6} & \textbf{95.97} & \textbf{81.82} & \textbf{93.49} & \textbf{88.96}  \\
            \hline
        \end{tabular}
    \end{minipage}
    \hfill % 水平填充，使两个 minipage 分开
    % --------------------
    % 表 2 (右侧)
    % --------------------
    \begin{minipage}[t]{0.45\textwidth}
        \centering
        \captionsetup{type=table} % 关键: 告诉 LaTeX 这是一个独立的表格
        \caption{\textbf{Ablation study of the three-stage training pipeline. We report AUC (\%) on five generalization benchmarks. }}
        \label{tab:abla-stage} % 更改了标签以防冲突
        \renewcommand\tabcolsep{2pt}
        \begin{tabular}{c|cccccc}
            \hline
            \multirow{2}*{Metrics} & \multicolumn{6}{c}{\underline{Test Set AUC}} \\       
              & CDF1 & CDF2 & DFDC & FFIW & WDF \\
            \hline
            stage1 & 96.77 & 94.03 & - & 90.89 & 87.63  \\
            stage2(w/sft)  & 91.53 & \textbf{95.8} & \textbf{81.58} & \textbf{92.37} & \textbf{89.13} \\
            stage3(VRAG-DFD) & \textbf{99.6} & \textbf{95.97} & \textbf{81.82} & \textbf{93.49} & \textbf{88.96}   \\
            \hline
        \end{tabular}
    \end{minipage}
    \hfill % 水平填充，使两个 minipage 分开

    % 注意：外层的 table* 环境不再需要 \caption 或 \label
    % 它现在只充当一个让两个表格并排的“浮动容器”
    
\end{table*}


\begin{table*}[htbp]
    \centering
    \scriptsize
    \renewcommand\arraystretch{1.2}

    % --------------------
    % 表 1 (左侧)
    % --------------------
    \begin{minipage}[t]{0.53\textwidth}
        \centering
        \captionsetup{type=table} % 关键: 告诉 LaTeX 这是一个独立的表格
        \caption{\textbf{
        Ablation study of retriever (AUC \%).
        'w/ CLIP-FFT' replaces our \texttt{Effort} retriever with a standard CLIP model full fine-tuned. 

        }}
        \label{tab:abla-retriveler} % 更改了标签以防冲突
        \renewcommand\tabcolsep{2pt}
        \begin{tabular}{c|cccccc}
            \hline
           \multirow{2}*{Metrics} & \multicolumn{5}{c}{\underline{Test Set AUC}} \\
            &  CDF1 & CDF2 & DFDC & FFIW & WDF \\
            \hline
            w/ CLIP-FFT & 90.12 & 87.07 & - & 86.4 & -  \\
            Effort & \textbf{95.97} & \textbf{81.82} & \textbf{93.49} & \textbf{88.96} & \textbf{99.6}  \\  
            \\
            \hline
        \end{tabular}
    \end{minipage}
    % --------------------
    % 表 2 (右侧)
    % --------------------
    \begin{minipage}[t]{0.53\textwidth}
        \centering
        \captionsetup{type=table} % 关键: 告诉 LaTeX 这是一个独立的表格
        \caption{\textbf{Effectiveness across different base MLLMs (AUC \%). 
        We show the performance of each model before (zero-shot) and after ('+ RAG-DFD (Ours)') applying our three-stage RAG-DFD pipeline. }}
        \label{tab:abla-MLLM} % 更改了标签以防冲突
        \renewcommand\tabcolsep{2pt}
        \begin{tabular}{c|cccccc}
            \hline
           \multirow{3}*{Metrics} & \multicolumn{5}{c}{\underline{Test Set AUC}} \\
            &  CDF1 & CDF2 & DFDC & FFIW & WDF \\
            \hline
            Qwen2.5VL-7b & 66 & 73.35 & 56.82 & 71.91 & 66.82  \\
            Qwen2.5VL+ours & 99.6 & 95.97 & 81.82 & 93.49 & 88.96  \\
            Intern3VL-8B & \textbf{66.33} & \textbf{72.06} & \textbf{57.19} & \textbf{70.86} & \textbf{65.75}  \\
            Intern3VL-8B + ours & \textbf{99.19} & \textbf{95.09} & \textbf{80.16} & \textbf{92.45} & \textbf{90} 
            
            \\
            \hline
        \end{tabular}
    \end{minipage}

    % 注意：外层的 table* 环境不再需要 \caption 或 \label
    % 它现在只充当一个让两个表格并排的“浮动容器”
    
\end{table*}
